Distributed k-Core Decomposition

Among the novel metrics used to study the relative importance of nodes in complex networks, k-core decomposition has found a number of applications in areas as diverse as sociology, proteinomics, graph visualization, and distributed system analysis and design. This paper proposes new distributed algorithms for the computation of the k-core decomposition of a network, with the purpose of (i) enabling the run-time computation of k-cores in "live" distributed systems and (ii) allowing the decomposition, over a set of connected machines, of very large graphs, that cannot be hosted in a single machine. Lower bounds on the algorithms complexity are given, and an exhaustive experimental analysis on real-world graphs is provided.

==> hadoop.tex <==
\section{Map-reduce}

The algorithm described above can be translated into a map-reduce algorithm.
The organization is based on two map-reduce jobs:
\begin{itemize}
\item The \emph{Reader} job takes a graph as input and transforms it in
a representation that is convenient for the job that follows. The input may be
formatted in many ways; here, we give an example where the graph is given as a
sequence of undirected edges (pairs of vertexes indentified by textual
strings). We transform it in a sequence of triplets $\langle \ID,
\INTEGER, \SET \langle ID \rangle \rangle$ which represent the vertex id, its
degree and the the set of vertexes connected to the vertex through an edge.
\item The \emph{Evaluator} job computes the k-shell index of all nodes; it is
applied several times, until all the nodes reach the correct value. In
each execution of the job, the input is given by a triplet $\langle \ID,
\INTEGER, \SET \langle ID \rangle \rangle$ (identical to the output of
Reader job); this time, the triplet represents the vertex id, the
current estimate of the k-shell index of the vertex id and a set of vertexes
to be notified. The mapper job creates a collection of “messages” that are
directed to the vertexes contained in the set, while the reducer collects
these messages and compute the new index, creating the triplets for the next
iteration.
\end{itemize}

The map-reduce implementation in Hadoop allows the slaves (those which
execute the map-reduce jobs) to communicate with the master; we use this
feature to communicate how many new estimates have been sent; the 
execution can stop as soon as there are no new estimates (or alternatively, 
when a very small number of new estimates have been produced, meaning that 
the process has almost converged).

\subsection{The Reader job}

The Reader job is extremely simple; it contains a mapper that doubles all the
incoming undirected edges in two directed edges. The reducer merges together
the edges originating from the same vertex (using set-theoretic operators to
discard duplicates) and counts the number of distinct istances. The final
output can thus be used as input from the next map-reduce job. To optimize
this job, we can either add a combiner (featuring the same behavior as the
reducer), or we can adopt the in-mapper combiner pattern. In the latter case,
a particular attention must be payed to avoid “out-of-memory” errors;
how to manage memory in an automated way is an open question.

\begin{algorithm}
\CLASS{\Mapper}{
  \METHOD{\Map(\TEXT $u$, \TEXT $v$)}{
    \Emit($\ID(u), (1, \{ \ID(v) \}$))\;
    \Emit($\ID(v), (1, \{ \ID(u) \}$))\;
  }
}
\BlankLine	
\CLASS{\Reducer}{
  \METHOD{\Reduce(\ID $u$, \INTEGER $d$, $\LIST\langle\SET\langle\ID\rangle\rangle\ L$)}{
    $\SET\langle\ID\rangle\ T \gets \emptyset$\;
    \ForEach{$S \in L$}{
      $T \gets T \cup S$\;
    }
    \Emit($u, (|T|, T)$)\;
  }
}	
\caption{The \emph{Reader} map-reduce job}
\label{alg:server}
\end{algorithm}

\subsection{The Evaluator job}

The first version of the Evaluator job is very simple:
it takes a triplet  $\langle \ID, \INTEGER, \SET \langle ID \rangle \rangle$
containing a vertex, its current shell-index estimate and its neighbor
set, computes the new shell-index set and emits a triplet in the same
format, with the new shell-index. In other words, the interesting data
(the shell-index estimate) and the graph structure are passed along
after each map-reduce iteration. This map-reduce job is repeated until
the termination condition is met.

For each vertex $u$, the mapper emits a “virtual message” to each neighbor
$v$ contained in the neighbor set of $u$; the key is given by the destination
vertex $v$ (to group together messages addressed to the same vertex), while the
message contains the identifier vertex $u$ and its current k-shell estimate.
Furthermore, it sends the estimate to itself as well. The reducer collect all 
this information, fill the $\Est$ array and the $\Index$ variable, and then 
calls the \ComputeIndex() method that has been used in the rest of the paper. 
It then emits a new triplet containing itself as a key, the new estimate and 
the set of neighbors, reconstructed from the virtual messages that have
been received.

\begin{algorithm}
\CLASS{\Mapper}{
  \METHOD{\Map(\ID $u$, \INTEGER $e$, $\SET\langle\ID\rangle\ S$)}{
    \ForEach{$v \in S$}{
      $\Emit(v, (u, e))$\;
    }
    $\Emit(u,(u,e))$\;
  }
}
\BlankLine	
\CLASS{\Reducer}{
  \METHOD{\Reduce(\ID $u$, $\LIST\langle \ID, \INTEGER\rangle\ L$)}{
    \ForEach{$(v,e) \in L$}{
      \eIf{$u = v$}{
      	$\Index \gets e$\;
      }{
        $\Est[v] \gets e$\;
      }
    }
    $k \gets \ComputeIndex(\Est, u, \Index)$\;
    $S \gets \{ v | (u,v,d) \in S \wedge u \neq v \}$\;
    \Emit($u, (k, S)$)\;
    \If{$k < Index$}{
      \Reporter.\Incr(“updates”)\;
    }
  }
}	
\caption{The \emph{Evaluator} map-reduce job (normal version)}
\label{alg:evaluator}
\end{algorithm}


\subsection{Grouping vertexes into clusters}

One important (and costly) step in the map-reduce paradigm  is the sorting operation
that assigns the keys to different reducers and guarantees that keys are seen
in order. The larger the number of keys, the heavier will be this step. In the
first version of our system, the number of keys is equal to the number of
vertexes.

A possible approach to reduce the number of keys is based on grouping vertexes
in larger units called \emph{clusters}. Each cluster contains a collection of
vertexes and manages the messages addressed to them. If a single reducer
manages a collection of vertexes, some steps of our algorithm can be
performed inside the cluster.

Requirements on how to
partition vertexes in clusters are as follows:
\begin{enumerate}
\item Each cluster \textbf{must} be uniquely identified by a unique \emph{cluster id};
\item Each cluster \textbf{must} contain a limited number of vertexes,
  because a cluster will be handled in-memory by a reducer, and this includes
  all the messages that are addressed to vertexes inside the cluster;
\item Each cluster should contain nodes that are \emph{close} to each 
  other, in order to avoid sending useless inter-cluster messages and
  maintain a large portion of the interactions intra-cluster.
\end{enumerate}

Some possible implementations are as follows:
\begin{itemize}
\item If the number $n$ of nodes is known in advance (or can be computed through
a map-reduce job), it is possible to hash each vertex id into a cluster id;
the number $c$ of different cluster id must be such that the expected number 
of vertexes id assigned to a cluster, $n/c$, can be easily handled in-memory
by the system;
\item If the number $n$ of nodes is known in advance and the nodes id are
assigned progressively between $0$ and the $n-1$, one can adopt the 
\emph{range partitioning} pattern~\cite{pattern}, in the hope that 
vertexes close to each other in graph are also close into the id space.
\item Potentially, a “smart” approach could be used to assign cluster ids
in a way that satisfies not only requirements (1) and (2) above, but also
requirement (3). 
\end{itemize}

To abstract our scheme from the specific mechanism used to assign vertexes
to clusters, we assume the existance of a function $c: V \rightarrow C$ such
that $c(u)$ is the cluster associated to the vertex $u$. While cluster
functions for the first and second methods are trivial, to implement the
first method we could assume that vertex ids carry information about clusters.

In the optimized algorithm, messages are addressed to the cluster containing
the destination vertex, instead of the vertex itself. To simplify code,
two types of messages are handled: \INDEX messages represent the current
estimates for vertexes that belongs to a particular cluster, while \UPDATE
messages are used to notify vertexes in a cluster about new estimates of
their neighbors.

The reducer manages all the information of a particular cluster; once
it has received all messages, it tries to improve the estimates by
simulating message exchanges among nodes belonging to the same cluster
(method \ImproveEstimate()). As before, the algorithm terminates when
no new updates are sent.

\begin{algorithm}
\CLASS{\Mapper}{
  \METHOD{\Map(\ID $u$, \INTEGER $e$, $\SET\langle\ID\rangle\ S$)}{
    \ForEach{$v \in S$}{
      $\Emit(c(v), (\UPDATE, v, u, e))$\;
    }
    $\Emit(c(u), (\INDEX, u, e)$\;
  }
}
\BlankLine	
\CLASS{\Reducer}{
  \METHOD{\Reduce(\CLUSTERID $c$, $\LIST\ L$)}{
  	$S \gets \emptyset$\;
    \ForEach{$(\INDEX,u,e) \in L$}{
      $\Est[u] \gets e$\;
      $S \gets S \cup \{ u \}$\;
    }
    \ForEach{$(\UPDATE,dst,src,e) \in L$}{
      $\Est[src] \gets e$\;
    }
    $\Changed \gets \ImproveEstimate(\Est, S)$\;
    \ForEach{$u \in S$}{
      $D \gets \{ src | (\UPDATE, dst, src, e) \in L \}$\;
      \Emit($u, (\Est[u], D)$)\;
    }
    \If{$\Changed$}{
      \Reporter.\Incr(“updates”)\;
    }
  }
}	
\caption{The \emph{Evaluator} map-reduce job (cluster version)}
\label{alg:evaluator-cluster}
\end{algorithm}


\begin{algorithm}
\caption{\ImproveEstimate($\INTEGER{[\,]}\ \Est$, $\SET\langle\ID\rangle\ S$)}	
$\Again \gets \TRUE$\;
$\Changed \gets \FALSE$\;
\While{$\Again$}{
  $\Again \gets \FALSE$\;
  \ForEach{$u \in S$}{
    $k \gets \ComputeIndex(\Est, u, \Est[u])$\;
    \If{$k < \Est[u]$}{
      $\Est[u] \gets k$\;
	  $\Again \gets \TRUE$\;
	  $\Changed \gets \TRUE$\;
    }
  }
}
\Return $\Changed$\;
\label{alg:improveEstimate}
\end{algorithm}

\subsection{Reducing the amount of messages - I}

Note that a message $(\UPDATE, dst, src, e)$ for cluster $c$ 
contains two kind of information: the new estimate of node $src$ is $e$, and
a neighbor of $src$ is $dst$. If $v$ and $w$ are both neighbor of $src$ and
they both belong to the same cluster $c$, the
information about the new estimate is repeated twice: $(\UPDATE, v,src, e)$
and $(\UPDATE, w,src, e)$. On the other, the information about the 
structure can be passed along through the schimmy pattern.

The modification in our code are simple: in the messages, we remove
information about $dst$ (the neighbor) and we just emit information
about the estimate. The mapper avoid to send the same message more
than once to the same cluster, by first computing the set of interested
clusters and then sending the message to them only once. In the reducer,
we use the schimmy pattern to reconstruct the structure of the network.
We asssume that the graph is divided in clusters, and that each cluster $c$
is associated with a neighbor map $N_c$ such that $N_c(u)$ is the set of
neighbors of $u$, provided that $c(u) = c$.

\begin{algorithm}
\CLASS{\Mapper}{
  \METHOD{\Map(\ID $u$, \INTEGER $e$, $\SET\langle\ID\rangle\ S$)}{
    $C \gets \emptyset$\;
    \ForEach{$v \in S$}{
      $C \gets C \cup \{ c(v) \}$\;
    }  
    \ForEach{$c \in C$}{
      $\Emit(c, (\UPDATE, u, e))$\;
    }
    $\Emit(c(u), (\INDEX, u, e)$\;
  }
}
\BlankLine	
\CLASS{\Reducer}{
  \METHOD{\Initialize()}{
    $R \gets \textsf{openGraphPartition}()$\;
  }
  \METHOD{\Reduce(\CLUSTERID $c$, $\LIST\ L$)}{
  	$S \gets \emptyset$\;
    \ForEach{$(\INDEX,u,e) \in L$}{
      $\Est[u] \gets e$\;
      $S \gets S \cup \{ u \}$\;
    }
    \ForEach{$(\UPDATE,src,e) \in L$}{
      $\Est[src] \gets e$\;
    }
    $\Changed \gets \ImproveEstimate(\Est, S)$\;
    \Repeat{$c' \neq c$}{
      $(c,N_c) \gets R.\Read()$\;
    }
    \ForEach{$u \in S$}{
      \Emit($u, (\Est[u], N_c(u))$)\;
    }
    \If{$\Changed$}{
      \Reporter.\Incr(“updates”)\;
    }
  }
}	
\caption{The \emph{Evaluator} map-reduce job (cluster,schimmy version)}
\label{alg:evaluator-cluster-schimmy}
\end{algorithm}




\subsection{Reducing the amount of messages}

It is immediate to note that this process is still extremely expensive, because it
involves all the vertexes in the graph, including those that have already
obtained the correct shell-index. Would it be possible to avoid all nodes
to be active?

\textbf{What follows, including the algorithm, is not correct}

The idea is the following: the set $S$ of vertexes in the triplet $(u,d,S)$
which constitutes the input is is not interpreted as the entire set of 
neighbor vertexes any more; instead, it only contains vertexes
that could be interested in a variation in the index of $u$. If the index
does not change, this set is empty. If the new index $k$ is smaller than
the previous one, this set includes all the neighbors whose current index 
is larger than $k$ -- in fact, the new index could cause a cascading 
change only in vertexes whose index is larger than $k$.

The mapper is similar to the previous one: but note that $S$ could be
empty, in which case the only information which is passed to the next
stage is the current index.

The reducer is different; first of all, we applied the schimmy pattern,
meaning that the graph structure is opened in the initializer and read
(but not emitted) at each reducing phase. The current index is obtained from
the set of “messages” produced by the mapper. The neighbor set $N$ of $u$
is read from the partition file. Then, variable $\Est$ is first initialized
by putting $\Index$ in all entries; then the values which are received
from other nodes are memorized value. If the new value is smaller than
the previous one, we generate a new message.

Note that in a real implementation, a partitioner must also be introduced
and the number of reducers must be specified. The output of each reducer
must be stored in a separate file, one per reducer, in order to use
the schimmy pattern in the next map-reduce job. How this can be done?


Problem: what happens if the information that could change the index 
are received at different moments? We risk to miss some changes - the
algorithm is not correct.

\begin{algorithm}
\CLASS{\Mapper}{
  \METHOD{\Map(\ID $u$, \INTEGER $d$, $\SET\langle\ID\rangle\ S$)}{
    \ForEach{$v \in S$}{
      $\Emit(v, (u, d))$\;
    }
    $\Emit(u,(u,d))$\;
  }
}
\BlankLine	
\CLASS{\Reducer}{
  \METHOD{\Initialize()}{
    $R \gets \textsf{openGraphPartition}()$\;
  }
  \METHOD{\Reduce(\ID $u$, $\LIST\langle \ID, \INTEGER\rangle\ S$)}{
    \ForEach{$(v,d) \in S$}{
      \If{$u = v$}{
    	$\Index \gets d$\;
      }
    }
    \Repeat{$u \neq v$}{
      $(v,N) \gets R.\Read()$\;
    }
    \lForEach{$v \in N$}{$\Est[v] \gets \Index$\;}
    \lForEach{$(u,v,d) \in S$}{$\Est[v] \gets d$\;}
    $k \gets \ComputeIndex(\Est, u, \Index)$\;
    \eIf{$\Index = k$}{
      $\Emit(u, (\Index, \emptyset))$\;
    }{
      $S \gets \{ v | (u,v,d) \in S \wedge u \neq v \wedge k < \Est[v] \}$\;
      $\Emit(u, (\Index, S))$\;
      \Reporter.\Incr(“updates”)
    }
  }
}	
\caption{The \emph{index-evaluation} map-reduce job (optimized version)}
\label{alg:server}
\end{algorithm}



